Russia's Ruble during the onset of the Russian invasion of Ukraine in early 2022: The role of implied volatility and attention

The onset of the Russo-Ukrainian crisis has led to the rapid depreciation of the Russian ruble. In this study, we model intraday price fluctuations of the USD/RUB and the EUR/RUB exchange rates from the $1^{st}$ of December 2021 to the $7^{th}$ of March 2022. Our approach is novel in that instead of using daily (low-frequency) measures of attention and investor's expectations, we use intraday (high-frequency) data: google searches and implied volatility to proxy investor's attention and expectations. We show that both approaches are useful in predicting intraday price fluctuations of the two exchange rates, although implied volatility encompasses intraday attention.

==> tables/table_2.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.5} 
\footnotesize

\caption{Correlation between price fluctuations and attention measures}
\label{table_2}

\begin{tabular}{cccccccc}
\toprule
                &             & \textbf{V1} & \textbf{V2} & \textbf{V3} & \textbf{V4} & \textbf{V5} & \textbf{V6} \\
                \midrule
$ln RV$              & \textbf{V1} & --          & 0,650       & 0,810       & 0,680       & 0,260       & 0,840       \\
General market ($ln$)  & \textbf{V2} & 0,650       & --          & 0,720       & 0,690       & 0,140       & 0,750       \\
Ruble ($ln$)           & \textbf{V3} & 0,830       & 0,720       & --          & 0,780       & 0,250       & 0,930       \\
Russian economy ($ln$) & \textbf{V4} & 0,680       & 0,670       & 0,770       & --          & 0,160       & 0,780       \\
$\Delta ln IV$      & \textbf{V5} & 0,360       & 0,220       & 0,340       & 0,240       & --          & 0,180       \\
$ln IV$             & \textbf{V6} & 0,830       & 0,740       & 0,930       & 0,770       & 0,240       & --  \\ 
\bottomrule
\multicolumn{8}{l}{\tiny{\parbox{0.8\linewidth}{\vspace{2pt}\textit{
Notes: Pearson's correlation coefficients between variables from the USD/RUB foreign exchange market correspond to the upper triangular, while values in the lower triangular correspond to the EUR RUB foreign exchange market variables.
}}}}  
\end{tabular}
\end{table}
